IRMaGiC: Extending Luminous Red Galaxy Selection into the Infrared with Joint Rubin Observatory's Large Survey of Space Time and Roman's High Latitude Imaging Survey

We introduce IRMaGiC, an algorithm built based on RedMaGiC desgined to enhance the selection of Luminous Red Galaxies (LRGs) across the redshift range $1 \leq z \leq 2$. We show that this method extends the capabilities of the redMaGiC algorithm by applying it to simulated photometric data from the Vera C. Rubin Observatory's Legacy Survey of Space and Time (LSST) and the Nancy Grace Roman Space Telescope's High Latitude Wide Area Survey (HLWAS). By integrating infrared band coverage from Roman HLWAS with LSST's optical bands, IRMaGiC enables red-sequence calibration at higher redshifts. We demonstrate that IRMaGiC reduces scatter and bias in photometric redshift estimates for LRGs at higher redshift, providing more accurate redshift assessments compared to existing methods. Our findings suggest that incorporating infrared data can considerably improve the selection and redshift estimation of LRGs at higher redshift, offering substantial benefits for future cosmological surveys.

==> author.tex <==
\author[0000-0001-9557-9171]{Zhiyuan Guo}
\affiliation{Department of Physics, Duke University, Durham, NC 27708, USA}

\author[0000-0003-2035-2380]{C. W. Walter}
\affiliation{Department of Physics, Duke University, Durham, NC 27708, USA}

\author[0000-0001-9376-3135]{Eli S. Rykoff}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology, 
P.O. Box 2450, Stanford University, Stanford, CA 94305, USA}

\author{The LSST Dark Energy Science Collaboration}


==> sections/outline.tex <==
\section{Outline} 
General outline
\begin{enumerate}
    \item Intro
    \item Data
    \begin{itemize}
        \item DC2 catalog (\textbf{photometric})
        \item Roman image simulation (\textbf{photometric})
        \item Truth and detection catalog
        \item Roman grism simulation (\textbf{spectroscopic})
        \item DC2 and Roman cross-matching (assumption of clear star and galaxy speration)
    \end{itemize}
    \item Method
     \begin{itemize}
         \item \st{Algorithm overview}
         \item \st{Seed Galaxy selection}
         \item \st{Red sequence template}
         \item \st{Roman Grism efficiency}
         \item \st{Overlapping area scaling}
         \item \st{Redshift estimation}
         \item \st{selection criteria}
         \item \st{Chi2 discussion}
         \item \st{photo-z afterburner}
         
     \end{itemize}
    \item Results
    \begin{itemize}
        \item \st{Photo-z performance}
        \item \st{Compare with DC2 photo-z}
        \item \st{Increasing overlapping area results.}
        \item Comparison with ANN photoz in DC2?
    \end{itemize}
    \item Summary
    \item Plots
    \begin{itemize}
        \item DC2 Roman simulation region compare?
        \item red galaxies selection color-color plot
        \item selection results: color vs redshift all vs selected red galaxies.
        \item DC2 + Roman RedMaGiC plot
        
        
    \end{itemize}
\end{enumerate}

\newpage
